Decentralized Fictitious Play in Near-Potential Games with Time-Varying Communication Networks

We study the convergence properties of decentralized fictitious play (DFP) for the class of near-potential games where the incentives of agents are nearly aligned with a potential function. In DFP, agents share information only with their current neighbors in a sequence of time-varying networks, keep estimates of other agents' empirical frequencies, and take actions to maximize their expected utility functions computed with respect to the estimated empirical frequencies. We show that empirical frequencies of actions converge to a set of strategies with potential function values that are larger than the potential function values obtained by approximate Nash equilibria of the closest potential game. This result establishes that DFP has identical convergence guarantees in near-potential games as the standard fictitious play in which agents observe the past actions of all the other agents.

==> conclusion.tex <==
% !TEX root = Control in state-based anti-coordination network games.tex

We considered the control of players' learning processes in a population to influence the emergent outcome in the context of anti-coordination network games. With the goal to promote maximum anti-coordination with minimum effort, we developed computationally tractable methods that determine when to control which players, and how to control them. An algorithm that sequentially selected players according to their influence in promoting anti-coordination in the future performed well in random networks with arbitrary population sizes.

%In this paper, we studied state-based anti-coordination network games where the players follow distributed learning dynamics. We formulated an optimal control problem for finding the minimum number of players to control that ensure the dynamics converge to maximum possible disagreement. We characterized the optimal policies for a line network for a range of payoff parameters, and find in some cases, cascades of decision-making can be leveraged to minimize control effort. For general networks, we proposed a greedy algorithm that computes a feasible, though often suboptimal, control policy to the problem, and evaluated its effectiveness on random bipartite networks through numerical simulations.


%Developing algorithms that achieve optimal behavior while conforming with the computational and informational limitations of the players is of interest given the ubiquity of noncooperative interactions that arise among actors in networked systems, e.g., energy, communication \cite{Bacci_et_al_2016} or autonomous systems \cite{marden2009cooperative}. Game theoretic learning algorithms are tractable decentralized models for decision-making in networked systems. These algorithms while accounting for local information access \cite{Swenson_et_al_2014} and coupled action spaces \cite{yi2017distributed} restrict attention to particular classes of games, e.g., aggregative \cite{parise2015network}, potential \cite{swenson2018distributed}, convex \cite{scutari2010convex}, to guarantee convergence to individually optimal behavior, i.e., a Nash equilibrium action profile. 
%
%A Nash equilibrium is optimal from the perspective of players. However, it can be inefficient and undesired at the system level. A canonical example of this is the tragedy of the commons which describes the phenomenon in which selfish learning behavior leads to the worst possible outcome for the entire population \cite{hardin1968tragedy}. Given the possibility of emergence of undesired outcomes, it is of interest to characterize the inefficiency of Nash equilibria \cite{marden2014generalized}, design payoffs prior to start of the game \cite{Li_Marden}, or develop incentive mechanisms given predetermined payoffs \cite{riehl2018incentive} in order to achieve system-wide desired outcomes. 
%
%In this paper, we consider an incentive mechanism with the goal to induce anti-coordination among players in a state-based network anti-coordination game by controlling a small number of players. In a state-based network anti-coordination game, players belong to one of two possible states. We assume there is a preferred selfish action, e.g., defecting in prisoners' dilemma, in the absence of any neighboring players. A player's payoff decreases as more of its neighbors belonging to the opposite state take the preferred action (Section \ref{sec:model}). These games can be used to model individual behavior during the spread of an epidemic in a population where the states are healthy and sick individuals, the actions represent the level of precautionary measures taken, and payoffs capture the risk of disease transmission to healthy from sick individuals \cite{eksin2017disease}. In these games two neighboring players anti-coordinate when at least one of the players do not take the selfish action, e.g., not taking  precautionary measures during an epidemic.
%
%We formulate the minimum player control for anti-coordination problem as a mixed integer program where the decision variables include which players to control, and how to control them (Section \ref{sec:MPCAC}). We assume players follow learning dynamics based on a decentralized algorithm that mimics the process of iterated elimination of strictly dominated actions in the absence of any control \cite{Fudenberg_Levine_1998}. We find a feasible policy that upper bounds the optimal policy by solving a minimum cardinality vertex covering problem on a reduced bipartite network (Theorem \ref{thm_vertex_cover}). In general, this policy is not optimal if there exists a way to cause cascades of anti-coordination among multi-hop neighbors via the learning dynamics by only controlling a few players. We characterize the optimal policy on a line network of arbitrary size for every possible payoff constant (Section \ref{sec:benchmark_optimal}). The optimal policy exhibits use of cascades to achieve anti-coordination. We also propose a greedy algorithm that finds a feasible, though often suboptimal, solution by sequentially disconnecting the player with the most active links in the network. We assess the algorithm in numerical experiments on random bipartite networks (Section \ref{sec:greedy}).
